Mellin-Barnes Integrals: A Primer on Particle Physics Applications

We discuss the Mellin-Barnes representation of complex multidimensional integrals. Experiments frontiered by the High-Luminosity Large Hadron Collider at CERN and future collider projects demand the development of computational methods to achieve the theoretical precision required by experimental setups. In this regard, performing higher-order calculations in perturbative quantum field theory is of paramount importance. The Mellin-Barnes integrals technique has been successfully applied to the analytic and numerical analysis of integrals connected with virtual and real higher-order perturbative corrections to particle scattering. Easy-to-follow examples with the supplemental online material introduce the reader to the construction and the analytic, approximate, and numeric solution of Mellin-Barnes integrals in Euclidean and Minkowskian kinematic regimes. It also includes an overview of the state-of-the-art software packages for manipulating and evaluating Mellin-Barnes integrals. These lecture notes are for advanced students and young researchers to master the theoretical background needed to perform perturbative quantum field theory calculations.

==> arxiv-pack <==
#!/bin/sh
# Build a self-contained arXiv source package: arxiv-source.tar.gz
#
# WHY THIS EXISTS
#   arXiv compiles without -shell-escape, so minted cannot run pygmentize
#   during arXiv's build. The solution for arXiv TeX Live 2023 (minted v2)
#   is the "frozen cache" workflow:
#     1. stage a copy of the source
#     2. build it once locally with [finalizecache] + -shell-escape; this
#        renames the hash-named cache files to listing1.pygtex ... listingN.pygtex
#     3. switch the staged copy to [frozencache] and verify that it compiles
#        WITHOUT -shell-escape (i.e. like arXiv does)
#     4. strip build artifacts (keeping _minted-bookv2/ and bu*.bbl) and tar
#
# The archive is FLAT: all files sit at the root of the tarball (no wrapper
# directory). arXiv finds the base file in a subdirectory too, but it then
# compiles "from the root of the submission directory" -- and pdfTeX resolves
# \input/\include/\includegraphics relative to the working directory, so a
# wrapper directory would break every relative path in this book.
#
# SUBMISSION NOTES
#   - select "TeX Live 2023" at submission time (NOT the default 2025:
#     TL2025 ships a rewritten minted v3 with an incompatible cache format)
#   - select processor "pdflatex"
#   - the package ships bu*.bbl on purpose: one .bib entry cites another
#     (the AMBRE entry cites Dubovyk:2015yba), so the .bbl must be present
#     for arXiv's single bibtex pass to see all citations.
#
# Requires locally: pdflatex, bibtex, pygmentize on PATH.
set -e
cd "$(dirname "$0")"

rm -rf arxiv-source
mkdir -p arxiv-source

# ---- 1. stage a copy of the source (flat: files at the archive root) --------
tar cf - \
    --exclude './arxiv-source' \
    --exclude './arxiv-source.tar.gz' \
    . | (cd arxiv-source && tar xf -)

cd arxiv-source

# ---- 2. freeze the minted cache (needs shell-escape + pygmentize) ----------
sed -i '' 's/^\\usepackage{minted}$/\\usepackage[finalizecache]{minted}/' bookv2.tex
pdflatex -interaction=nonstopmode -shell-escape bookv2.tex
for i in bu*.aux; do bibtex "$i" || true; done
pdflatex -interaction=nonstopmode -shell-escape bookv2.tex
pdflatex -interaction=nonstopmode -shell-escape bookv2.tex
if grep -q '^!' bookv2.log; then echo "ERROR: finalizecache build failed"; exit 1; fi

# ---- 3. switch to frozencache, verify WITHOUT shell-escape (arXiv env) -----
sed -i '' 's/^\\usepackage\[finalizecache\]{minted}$/\\usepackage[frozencache]{minted}/' bookv2.tex
rm -f ./*.aux bookv2.out bookv2.toc bookv2.idx bookv2.thm
# (keep bu*.bbl -- shipped with the package)
pdflatex -interaction=nonstopmode -no-shell-escape bookv2.tex
for i in bu*.aux; do bibtex "$i" || true; done
pdflatex -interaction=nonstopmode -no-shell-escape bookv2.tex
pdflatex -interaction=nonstopmode -no-shell-escape bookv2.tex
if grep -q '^!' bookv2.log; then echo "ERROR: no-shell-escape verification failed"; exit 1; fi
if grep -qE "Citation .* undefined|There were undefined references" bookv2.log; then
    echo "ERROR: undefined citations in no-shell-escape build"; exit 1
fi

# ---- 4. strip build artifacts (keep minted cache + .bbl), tar ---------------
rm -f ./*.aux ./*.blg ./*.log ./*.out ./*.toc ./*.lof ./*.lot
rm -f ./*.idx ./*.ind ./*.ilg ./*.thm ./*.synctex.gz
rm -f ./*.pyg
rm -f ./bookv2.pdf
cd ..

tar czf arxiv-source.tar.gz -C arxiv-source .
rm -rf arxiv-source
echo "-------------------------------------------------------------------"
echo "Created arxiv-source.tar.gz  ($(du -h arxiv-source.tar.gz | cut -f1))"
echo "Verify the minted freeze is in the package:"
tar tzf arxiv-source.tar.gz | grep -E "_minted|bookv2.tex|\.bbl$" | head -15


==> clean <==
#!/bin/sh
# Remove all build artifacts, leaving only the source files.
#
#   ./clean          (or:  ./run clean)
#
# What gets removed:
#   - LaTeX/bibtex aux files:  *.aux  bu*.bbl  bu*.blg
#   - output/log files:        *.log  *.out  *.toc  *.lof  *.lot  *.idx
#                              *.ind  *.ilg  *.thm  *.synctex.gz  bookv2.pdf
#   - minted highlight cache:  _minted-bookv2/
#   - arXiv staging dir:       arxiv-source/   (the tarball is kept)
#   - editor/OS cruft:         .DS_Store  *.swp  *~  *.bak
#
# Everything under FIGS/, MBambre/ and bibs/ is kept (that is content).
set -e
cd "$(dirname "$0")"

# LaTeX / bibtex auxiliary outputs (top level only)
rm -f ./*.aux ./*.bbl ./*.blg
rm -f ./*.log ./*.out ./*.toc ./*.lof ./*.lot
rm -f ./*.idx ./*.ind ./*.ilg ./*.thm ./*.synctex.gz
rm -f ./*.pyg ./*.pygstyle

# the built PDF
rm -f ./bookv2.pdf

# minted highlight cache
rm -rf ./_minted-bookv2

# arXiv packaging staging dir (the tarball is a deliverable, so it is kept;
# run arxiv-pack to regenerate it). Delete arxiv-source.tar.gz manually if wanted.
rm -rf ./arxiv-source

# editor / OS cruft
find . \( -name '.DS_Store' -o -name '*.swp' -o -name '.#*' \
          -o -name '*~' -o -name '*.bak' \) -type f -delete

echo "Cleaned. Remaining files:"
ls -1A


==> foreword.tex <==
%%%%%%%%%%%%%%%%%%%%%%foreword.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample foreword
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\foreword

%% Please have the foreword written here
This Foreword was supposed to be, as planned in the Synopsis, written by our friend Dr. Tord Riemann. Unfortunately, he left us on 2nd April 2021, before we managed to finish the work. 

As the authors of this book we  are thankful to Tord for his permanent support and encouragement for writing up the notes on Mellin-Barnes integrals. 

\begin{figure}
    \centering 
%    \label{}
 %{\small}\\
%\includegraphics[height=3cm]{figs/Mellin}
 \includegraphics[height=3cm]{figs/CCSepOct21_OBITS_Riemann-635x512.jpg}\\
%\hspace*{5cm}  {\small }
 \caption*{Dr. Tord Riemann, 1951-2021, \colbref{https://cerncourier.com/a/tord-riemann-1951-2021/}. Photo thanks to Dr. Sabine~Riemann.}
\end{figure}

We dedicate this book to the memory of Dr. Tord Riemann. 

\vspace{\baselineskip}
\begin{flushright}\noindent
Place, month year\hfill {\it Authors}\\
\end{flushright}




==> glossary.tex <==
%%%%%%%%%%%%%%%%%%%%%%acronym.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample list of acronyms
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\Extrachap{Glossary}


Use the template \emph{glossary.tex} together with the Springer document class SVMono (monograph-type books) or SVMult (edited books) to style your glossary\index{glossary} in the Springer layout.


\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

==> preface.tex <==
%%%%%%%%%%%%%%%%%%%%%%preface.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample preface
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\preface

%% Please write your preface here
%%Customarily \textit{acknowledgments} are included as last part of the preface.
%}}}
%\begin{flushright}
%{\it Today in the sciences, books are usually either texts or retrospective reflections upon one aspect or another of the scientific life. The scientist who writes one is more likely to find his professional reputation impaired than enhanced. }\newline 
%Thomas~S.~Kuhn `The structure of scientific revolutions'
%\end{flushright}

\vspace{-3cm}
\begin{figure}
    \centering 
%    \label{}
 %{\small}\\
%\includegraphics[height=4cm]{figs/Mellin}
\includegraphics[height=4.5cm]{FIGS/eMuseumPlusMellin_frame.jpg}
 \includegraphics[height=4.5cm]{FIGS/Ernest_William_Barnes.jpg}\\
%\hspace*{5cm}  {\small }
 \caption*{On the left: Hjalmar Mellin (1854-1933) Finnish mathematician, Helsinki University of Technology. \copyright{}
 Atelier Charles Rüs \& Co., Hjalmar Mellin, Ident.Nr. 1992,32/003a.024, Kunstbibliothek, Staatlichen Museen zu Berlin under CC BY-NC-SA 3.0 DE,  \colbref{http://www.smb-digital.de/eMuseumPlus}.\\
 On the right: Ernest William Barnes (1874-1953)  British mathematician, liberal 
 theologian and bishop. {\copyright Foto:  \colbref{https://en.wikipedia.org/wiki/Ernest\_Barnes}}.} %\colbref{https://en.wikipedia.org/wiki}}.
\end{figure}

This book is about the mathematical basics of {\textit{Mellin-Barnes}} integrals,
however, it is motivated by the practical needs of precision calculations in particle physics. 

In modelling physical phenomena, we aim at predictability and exactness. 
In particle physics a compelling model exists, commonly called the Standard Model (SM), which describes elementary particles and their interactions.  We know since the 1960's that gauge interactions, 
mathematically based on a product of $U(1)$, $SU(2)$ and $SU(3)$ groups, describe the electromagnetic, weak and strong forces. We know the charges, spins, C and P parities, as well as the masses of 
elementary particles. We understand how fermions and bosons interact by chiral weak interactions 
and we understand the dynamics of the quarks and gluons that partake in the strong interaction. 
The SM describes innumerable physical phenomena observed in the laboratory and the cosmos, linking present-day experiments with the first $10^{-11}$ second of the Universe. 
Looking at the list of Nobel laureates in Physics, many of them are connected with particle physics. 
Their awards speak to the appreciation of the Standard Model theory builders and to the enormous efforts 
made to confirm the SM structure and predictions experimentally.
%, with elusive effects defined within the model (QCD theory, neutrinos, Higgs boson). 
 
The SM is surprisingly precise in its predictions and complete in the sense that all of its theorized 
elementary particles have now been observed. %All its elementary particles have been discovered, and the model describes very well the observed effects.
The last missing piece of the SM, the Higgs boson was discovered in 2012. This discovery was made 
possible by the construction of the LHC accelerator {and} the ATLAS and CMS detectors, whose designs 
were guided by theoretical predictions based on the SM. Thus, we now believe that we can answer the  theoretical question dating from the 1960s: "what gives mass to the electroweak bosons?".  

{\textit{However, this achievement does not stop the need for further exploration!}}
%This discovery also completed the set of particles and interactions that form the Standard Model (SM). 

First, does the ${\rm 125 GeV/c^2}$ particle that was discovered really play the role which theory says it does? Second, several unanswered mysteries call for new phenomena beyond the SM: (i) the apparent 
presence of dark matter in the Universe; (ii) the matter-antimatter asymmetry of the Universe; and (iii) 
the existence and pattern of neutrino masses to name three outstanding ones. Although the list of 
issues to be explored in the future is long\footnote{\label{briefbook} Physics Briefing Book : Input for the European Strategy for Particle Physics Update 2020,
Richard Keith Ellis et al., CERN-ESU-004,
\href{http://arxiv.org/abs/arXiv:1910.11775}{arXiv:1910.11775}.}, there is at present no clear guidance on the energy scale or strength of the new phenomena. However since the SM is complete, there is no freedom in its predictions and any observed deviation would be a discovery and a precious pointer 
into the unknown. 
An ambitious program of precision Higgs and electroweak measurements is thus in order.
%, in Europe triggered by the European Strategy for Particle Physics Update 2020. 
%In this regard, SM predictions motivate which accelerators and detectors to construct and provide 
%a baseline to be compared with experimental data. 
%
%it ``calibrates'' what can be simulated and compared with experimental data. 
%Concerning lepton colliders we mean especially the FCC-ee project ...
%
%{\em However, collider physics needs more than experimental efforts: It needs Theory}. 
However, a well-prepared and well-motivated collider project requires precise theory input to guide 
the experiment and confront the results, thus optimizing the chances for significant scientific 
progress. Ever-increasing mathematical virtuosity is however required to reach the ever-improving 
level of experimental precision. 

{\textit{And this is a place where the theory and methods connected with Mellin-Barnes integrals described in the book enter. }}

To achieve the required precision of theoretical calculations, higher-order perturbative 
corrections in Quantum Field Theory must be calculated. This involves the computation of so-called 
multi loop Feynman integrals as well as phase space integrals. 
%\textit{Precision} is here a key word. 
However, currently there is no complete theory for Feynman integrals beyond one loop. This defines 
a challenge to theoreticians and calls for innovative methods and tools, both numerical and analytical.
%To extract tiny effects beyound the SM (BSM) from experiments we must measure more and more precisely and calculate corresponding measured observables with higher and higher accuracy. 
%From theoretical point of view in hunt for BSM effects in particle physics our main concern is about developing techniques and tools for precision observables measurements. For this exploration of advanced \textit{mathematics} is needed.
%And this is where we stand.

%Theoretical calculations in microscale must be precise, otherwise there is no way to extract tiny details connected with colliding particles, their creation and decays or indirect, virtual effects. 
This book focuses on one of these, the \textit{Mellin-Barnes} (MB) method. This method has been 
applied to real applications at the frontier of research and has proven to be one of very few 
ones which could solve so far untouchable problems of precision physics. 
%, which proved to be in frontier of real applications, as one of very few directions which can solve 
%so far untouchable regions of precision physics. 
The book provides a self-contained overview of the necessary elements of complex analysis and 
special functions, an easy-to-follow introduction to the subject of MB representations with 
hands-on examples and a comprehensive view on the analytical and numerical methods and tools
related to MB integrals. It should be a good starting point for learning and using the MB method 
in practical research.
%We plan to apply it to high energy collider calculations (LHC, ILC, FCC-ee, FCC-hh, GigaZ) as well low energy meson factory and intensity frontier experiments. 

%Though we focus on application of MB to collider physics it  can  serve also in other branches of physics. ...
%{\it Today in the sciences, books are usually either texts or retrospective reflections upon one aspect or another of the scientific life. The scientist who writes one is more likely to find his professional reputation impaired than enhanced}\footnote{
%Thomas~S.~Kuhn `The structure of scientific revolutions', The University of Chicago Press.}. 
 
 
\vspace{\baselineskip}
\begin{flushright}\noindent
Katowice, Cisownica, Budapest\hfill {\it Ievgen Dubovyk}\\
October 2022\hfill {\it Janusz Gluza}\\
\hfill {\it G\'abor Somogyi}
\end{flushright}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% OLD: COMMENTED OUT                                   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
%% Please write your preface here
%%Customarily \textit{acknowledgments} are included as last part of the preface.
%}}}
%\begin{flushright}
%{\it Today in the sciences, books are usually either texts or retrospective reflections upon one aspect or another of the scientific life. The scientist who writes one is more likely to find his professional reputation impaired than enhanced. }\newline 
%Thomas~S.~Kuhn `The structure of scientific revolutions'
%\end{flushright}

\begin{figure}
    \centering 
%    \label{}
 %{\small}\\
\includegraphics[height=3cm]{figs/Mellin}
 \includegraphics[height=3cm]{figs/Barnes}\\
%\hspace*{5cm}  {\small }
 \caption*{On left: Mellin, Hjalmar, 1854-1933, a Finnish mathematician, Helsinki University of Technology. On right: Barnes, Ernest, William, 1874-1953, a British mathematician, a liberal theologian and bishop.  Pictures source: \colbref{https://en.wikipedia.org/wiki}}.
\end{figure}

This book is about mathematical basics of {\textit{Mellin-Barnes}} integrals,
however, it is motivated by the physical needs of precision calculations in particle physics. 

In modelling physical phenomena, we aim at predictability and exactness. 
In particle physics a compelling model exists, commonly called the Standard Model, which describes elementary particles and their interactions.  We know from the sixties of the last century that gauge interactions describe electromagnetic, weak and strong forces, mathematically based on a product of $U(1)$, $SU(2)$ and $SU(3)$ groups. We know charges, spins, C and P parities, as well as masses of elementary particles. We understand how fermions and bosons interact by chiral weak interactions and understand quarks and gluons dynamics of strong interactions. 
The SM describes innumerable physical phenomena observed in the laboratory and the cosmos linking present-day experiments with the first $10^{-11}$ second of the Universe. 
Looking into Nobel prize winners in Physics, many of them are connected with particle physics. They were awarded to appreciate the Standard Model theory builders and enormous efforts to confirm SM structure and predictions experimentally.
%, with elusive effects defined within the model (QCD theory, neutrinos, Higgs boson). 
 
The SM model is surprisingly precise in predictions and complete. %All its elementary particles have been discovered, and the model describes very well the observed effects.  
The discovery of the Higgs boson in 2012, the last missing piece of the SM was made possible by building the LHC accelerator {and} the ATLAS and CMS detectors, whose design was guided by theoretical predictions based on the Standard Model (SM) of particle physics to answer a theoretical question dating from the 1960s: "what gives mass to the electroweak bosons?".  
%To explore further particle physics in understanding universe in micro and macro scales %(gravity, small neutrino masses, hierarchy problem, parity restoration, notion of extra dimensions and supergravity, cosmology with dark matter and dark energy problems) 
%new precision experiments are needed.  

{\textit{This achievement does not stop the need for further exploration.}}
%This discovery also completed the set of particles and interactions that form the Standard Model (SM). 

First, does the ${\rm 126 GeV/c^2}$ particle that was discovered really play the role which theory says it should? Secondly, several unanswered mysteries call for new phenomena beyond the SM: (i) dark matter; (ii) the matter-antimatter asymmetry of the Universe; (iii) the existence and pattern of neutrino masses. The list of issues to be explored at future is long\footnote{\label{briefbook} Physics Briefing Book : Input for the European Strategy for Particle Physics Update 2020,
Richard Keith Ellis et al., CERN-ESU-004,
\href{http://arxiv.org/abs/arXiv:1910.11775}{arXiv:1910.11775}.}.
There is no clear guidance on the scale of energy or strength of the new phenomena; however since the SM is complete, there is no freedom in its predictions, and any observed deviation would be a discovery and a precious pointer into the unknown. 
An ambitious program of precision Higgs and Electroweak measurements is thus in order, in Europe triggered by the European Strategy for Particle Physics Update 2020. 
The SM theory motivates which accelerators and detectors to construct and it ``calibrates'' what can be simulated and compared with experimental data. 
%Concerning lepton colliders we mean especially the FCC-ee project ...

%{\em However, collider physics needs more than experimental efforts: It needs Theory}. 
A well-prepared and well-motivated collider projects require the precise theory to guide the experiment and confront the results, thus optimizing the chances for significant scientific progress.  
Ever-increasing mathematical virtuosity is however required to reach the ever-improving level of experimental precision. 

{\textit{And this is a place where the theory and methods connected with Mellin-Barnes integrals described in the book enters. }}

To leverage precision of theoretical calculations, we need to explore higher-order perturbation Quantum Field Theory represented by Feynman integrals. 
%\textit{Precision} is here a key word. 
There is no complete theory for perturbation calculations of Feynman integrals beyond one loop. This defines a challenge to theoreticians and calls for innovative methods and tools which are both numerical and analytical.
%To extract tiny effects beyound the SM (BSM) from experiments we must measure more and more precisely and calculate corresponding measured observables with higher and higher accuracy. 
%From theoretical point of view in hunt for BSM effects in particle physics our main concern is about developing techniques and tools for precision observables measurements. For this exploration of advanced \textit{mathematics} is needed.
%And this is where we stand.

%Theoretical calculations in microscale must be precise, otherwise there is no way to extract tiny details connected with colliding particles, their creation and decays or indirect, virtual effects. 
We are focusing on one of them, the \textit{Mellin-Barnes} method, which proved to be in frontier of real applications, as one of very few directions which can solve so far untouchable regions of precision physics. It brings a self-contained overview of the necessary elements of complex analysis
and special functions,
easy-to-follow introduction with hands-on examples to the complex
analysis of Mellin-Barnes representations and comprehensive view on the analytical and numerical methods and tools
related to Mellin-Barnes integrals.
It should be a good starting point to learn and use the MB methods in research practice.
%We plan to apply it to high energy collider calculations (LHC, ILC, FCC-ee, FCC-hh, GigaZ) as well low energy meson factory and intensity frontier experiments. 

%Though we focus on application of MB to collider physics it  can  serve also in other branches of physics. ...
%{\it Today in the sciences, books are usually either texts or retrospective reflections upon one aspect or another of the scientific life. The scientist who writes one is more likely to find his professional reputation impaired than enhanced}\footnote{
%Thomas~S.~Kuhn `The structure of scientific revolutions', The University of Chicago Press.}. 
 
 
\vspace{\baselineskip}
\begin{flushright}\noindent
Place(s),\hfill {\it Ievgen Dubovyk}\\
month year\hfill {\it Janusz Gluza}\\
\hfill {\it Gabor Somogyi}
\end{flushright}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% END OF OLD: COMMENTED OUT                            %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi

==> run <==
#!/bin/sh
# Build the book. Requirements:
#   - pdflatex with -shell-escape (minted needs it)
#   - pygmentize on PATH (pip install pygments / brew install pygments)
#
# Bibtex is run TWICE: some .bib entries contain \cite commands in their
# note fields (e.g. the AMBRE homepage entry cites Dubovyk:2015yba). Those
# citations only appear in the aux file after the first .bbl has been
# processed, so a second bibtex pass is required for a complete .bbl.
#
# Note: bibtex exits 2 with "Repeated entry" warnings; that is harmless
# (duplicate keys across the shared .bib files are deduplicated, the first
# occurrence wins). The build succeeds regardless.
set -e
pdflatex -interaction=nonstopmode -shell-escape bookv2.tex
for i in bu*.aux; do bibtex "$i" || true; done
pdflatex -interaction=nonstopmode -shell-escape bookv2.tex
for i in bu*.aux; do bibtex "$i" || true; done
pdflatex -interaction=nonstopmode -shell-escape bookv2.tex
pdflatex -interaction=nonstopmode -shell-escape bookv2.tex
#rm bu*aux bu*blg all.toc all.aux all.out all.log


==> solutions.tex <==

\Extrachap{Solutions}

\section*{Problems of Chapter~\ref{intro}}

\begin{sol}{prob1}
The solution\index{problems}\index{solutions} is revealed here.
\end{sol}


\begin{sol}{prob2}
\textbf{Problem Heading}\\
(a) The solution of first part is revealed here.\\
(b) The solution of second part is revealed here.
\end{sol}


